Motion comfort and driver feel: An explorative study about their relation in remote driving

Teleoperation is considered as a viable option to control fully automated vehicles (AVs) of Level 4 and 5 in special conditions. However, by bringing the remote drivers in the loop, their driving experience should be realistic to secure safe and comfortable remote control.Therefore, the remote control tower should be designed such that remote drivers receive high quality cues regarding the vehicle state and the driving environment. In this direction, the steering feedback could be manipulated to provide feedback to the remote drivers regarding how the vehicle reacts to their commands. However, until now, it is unclear how the remote drivers' steering feel could impact occupant's motion comfort. This paper focuses on exploring how the driver feel in remote (RD) and normal driving (ND) are related with motion comfort. More specifically, different types of steering feedback controllers are applied in (a) the steering system of a Research Concept Vehicle-model E (RCV-E) and (b) the steering system of a remote control tower. An experiment was performed to assess driver feel when the RCV-E is normally and remotely driven. Subjective assessment and objective metrics are employed to assess drivers' feel and occupants' motion comfort in both remote and normal driving scenarios. The results illustrate that motion sickness and ride comfort are only affected by the steering velocity in remote driving, while throttle input variations affect them in normal driving. The results demonstrate that motion sickness and steering velocity increase both around 25$\%$ from normal to remote driving.

==> 04_Results05.tex <==
\subsection{Predicting RC and MS based on subjective assessment in ND and RD}

After having unravelled the relation of driver feel with motion comfort in ND and RD, unique models to predict RC (MDL$_{RC/{ND}}$ and MDL$_{RC/{RD}}$) and MS (MDL$_{MS/{ND}}$ and MDL$_{MS/{RD}}$) are developed using SA metrics as predictors. 
To not increase the models complexity or develop over-fitted models without capturing the proper relation between predictors and prediction values, the predictors are selected according to the previous section and the redundancies outlined through Table \ref{tab:subj_correlation}. 
More specifically, all level 1-2 metrics have not been considered as predictors since it was proved that they are redundant and they are highly related with the level 3 metrics. 
Therefore, the prediction models consider only the level 3 SA metrics as predictors.
The models also consider interactions between the predictors to improve the fitting and further unravel the impact of SAs metrics on motion comfort.
The developed models, using stepwise multiple regression in MATLAB 2021b, are presented in Table \ref{tab:regression_model2b}, while the predictor effects on RC and MS are illustrated in Figure \ref{fig:Effects_RC_MS}.

According to Table \ref{tab:regression_model2b}, MDL$_{RC/{ND}}$ and MDL$_{RC/{RD}}$ (i.e. the models to predict RC in ND and RD) are with high correlation and their prediction is of high significance, while the MDL$_{MS/{ND}}$ and MDL$_{MS/{RD}}$ predict MS with lower correlation and significance.
More specifically, the model predictions (MDL$_{RC/{ND}}$ and MDL$_{RC/{RD}}$) display high adjusted R$^2$ values from 0.83 to 0.99, and a p-values less than 0.001. 
This high prediction and accurate levels provided by MDL$_{RC/{ND}}$ and MDL$_{RC/{RD}}$ are in alignment with the correlation levels of each SA metric with RC (Table \ref{tab:RSquareOfCorrelation}).
At the same time, MDL$_{RC/{ND}}$ predicts MS in ND with adjusted R$^2$ around 0.53 and no significance (p-value = 0.136). 
Higher accuracy and significance was expected based on the satisfactory correlation of the SAs metrics with MS in ND (Table \ref{tab:RSquareOfCorrelation}).
On contrary to what was expected based on the same table, MS is predicted in RD (MDL$_{RC/{RD}}$) with much higher correlation and significance than in ND with an adjusted R$^2$ around 0.88 and p-value equal to 0.016. 

The predictors for the models are selected among all the SA metrics from Table \ref{tab:SA_Metrics} based on the redundancies identified before, considering only the Level 3 SA metrics at the end.
However, the stepwise linear regression method removed predictors, that are not significant and do not increase the model's regression (R$^2$) reasonably, to deliver the optimal model. 
Eventually, the MDL$_{RC/{ND}}$ considers all the Level 3 SAs metrics as predictors, while it includes only three interactions between four of the predictors (SA12,SA22,SA31 and SA32).
Meanwhile, MDL$_{RC/{RD}}$ do not consider SA11 and SA31 as predictors.
The removal of the first is not in accordance to the ample correlation of the metric with RC (Table \ref{tab:RSquareOfCorrelation}), whereas the removal of the latter was expected.
Regarding interactions, the model includes only two interactions between the same terms with MDL$_{RC/ND}$, except from SA12.
% \textcolor{red}{Finally, in both models, the already high correlation of the SA metrics with RC, as shown in Table \ref{tab:RSquareOfCorrelation}, allowed the two models (MDL$_{RC/ND}$ and MDL$_{RC/RD}$) to achieve high predictability of RC and great significance levels with limited number of interaction terms.} 

\input{04_Results_table2.tex}

% Overall subjective steering feel (SA0)
\begin{figure*}[h!]
\centering
\begin{subfigure}{0.45\linewidth}
  \centering 
  \includegraphics[width=\linewidth]{Pics/Effects/Effects_Level2_RC.pdf}
  \caption{}
  \label{fig:Effects_Level2_RC}
\end{subfigure}
\hfill
\begin{subfigure}{0.45\linewidth}
  \centering 
  \includegraphics[width=\linewidth]{Pics/Effects/Effects_Level2_MS.pdf}
  \caption{}
  \label{fig:Effects_Level2_MS}
\end{subfigure}
\caption{The effects of the different predictors (Level 3 SAs metrics) in the multiple regression model for the prediction of (a) RC and (b) MS in normal driving (ND) and remote driving (RD) scenarios. The horizontal line through an effect value indicates the 95$\%$ confidence interval for the effect value.} \label{fig:Effects_RC_MS}
\end{figure*}

The effect of the selected predictors in both models is illustrated in Figure \ref{fig:Effects_Level2_RC}, where the spread of the horizontal lines represent the 95$\%$ confidence interval.
Regarding the captured effect, first of all, the confidence level for all cases is very high based on the low spread in most of the predictors' effect.
The two models are able to capture the potential contradictory relation of SA metrics with RC in RD and ND, as identified previously. 
Although, in some cases, the effect is opposing to what has been identified.
More specifically, similarly with Figure \ref{fig:RC_MS_SA12_S}, the effect of SA12 on the RC prediction of MDL$_{RC/{RD}}$ and MDL$_{RC/{ND}}$ is in conflict. 
In MDL$_{RC/{ND}}$, the change in SA12 has a negative effect on RC (i.e., RC decrease), whereas in MDL$_{RC/{RD}}$ the same change leads to a positive effect (i.e., RC increase). 
On the other hand, the effect of SA32 on the prediction of RC by MDL$_{RC/{ND}}$ and MDL$_{RC/{RD}}$ opposes to what was identified in Figure \ref{fig:RC_MS_SA32_S}. 
The change of SA32 has a positive effect on RC in ND (MDL$_{RC/ND}$), while the effect is negative in RD (MDL$_{RC/RD}$). 
The opposite effect is captured in Figure \ref{fig:RC_MS_SA32_S}.
Similarly, SA21, which was expected to have the same behaviour as SA20 (Figure \ref{fig:RC_MS_SA20_S}) based on their high correlation ($\rho_{SA20,SA21}$=0.96), is also illustrating contradictory effect.
% The effect of a predictor represents is calculated by changing the predictor value while averaging out the effects of the other predictor.



==> 04_Results_table2.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{table*}[h!]
% \caption{Paired-sample t-test to identify if the RC, MS, SV and TI data in ND and RD come from a normal distribution with mean value equal to zero.}    
% \begin{tabular}{|cc|cccc|cccc|}
% \hline
% \multicolumn{2}{|c|}{{\color[HTML]{330001} }}                                            & \multicolumn{4}{c|}{}                                                                                                                                                                                          & \multicolumn{4}{c|}{}                                                                                                                                                                                          \\
% \multicolumn{2}{|c|}{\multirow{-2}{*}{{\color[HTML]{330001} }}}                          & \multicolumn{4}{c|}{\multirow{-2}{*}{\textbf{Normal driving}}}                                                                                                                                                 & \multicolumn{4}{c|}{\multirow{-2}{*}{\textbf{Remote driving}}}                                                                                                                                                 \\ \hline
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{}                                      &                                     & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{}                                      &                                     \\
% \multicolumn{1}{|c|}{\multirow{-2}{*}{\textbf{Level}}} & \multirow{-2}{*}{\textbf{Term}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{R$^2$}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$P$}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Predictors}}} & \multirow{-2}{*}{\textbf{Terms}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{R$^2$}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{$P$}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Predictors}}} & \multirow{-2}{*}{\textbf{Terms}} \\ \hline
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Intercept}                             & 2.686                               & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Intercept}                             & 2.953                               \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01}                                  & -1.109                              & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01}                                  & -0.414                              \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA10}                                  & 0.134                               & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA10}                                  & -0.855                              \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA20}                                  & 0.870                               & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA20}                                  & 0.779                               \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{0.775}}       & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA30}                                  & -0.417                              & \multicolumn{1}{c|}{\multirow{-5}{*}{0.601}}       & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA30}                                  & -                                   \\ \cline{3-3} \cline{5-7} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA10}                             & -0.347                              & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA10}                             & 0.363                               \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA20}                             & -                                   & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA20}                             & -0.295                              \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA30}                             & 0.706                               & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA30}                             & -                                   \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA10*SA20}                             & 0.355                               & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA10*SA20}                             & -                                   \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 & \multirow{-10}{*}{\textbf{RC}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{0.474}}       & \multicolumn{1}{c|}{\multirow{-10}{*}{0.132}}          & \multicolumn{1}{c|}{SA20*SA30}                             & -0.621                              & \multicolumn{1}{c|}{\multirow{-5}{*}{0.379}}       & \multicolumn{1}{c|}{\multirow{-10}{*}{0.092}}          & \multicolumn{1}{c|}{SA20*SA30}                             & -                                   \\ \cline{2-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Intercept}                             & 1.290                               & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Intercept}                             & 3.026                               \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01}                                  & -0.657                              & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01}                                  & 1.264                               \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA10}                                  & 0.341                               & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA10}                                  & -1.800                              \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA20}                                  & 0.615                               & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA20}                                  & -0.569                              \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{\multirow{-5}{*}{0.809}}       & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA30}                                  & -0.559                              & \multicolumn{1}{c|}{\multirow{-5}{*}{0.833}}       & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA30}                                  & -0.133                              \\ \cline{3-3} \cline{5-7} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA10}                             & -0.109                              & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA10}                             & 1.045                               \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA20}                             & -                                   & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA20}                             & -0.498                              \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA30}                             & 0.315                               & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA01*SA30}                             & -0.875                              \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{}                                 &                                 & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA10*SA20}                             & -                                   & \multicolumn{1}{c|}{}                              & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA10*SA20}                             & -0.455                              \\ \cline{5-6} \cline{9-10} 
% \multicolumn{1}{|c|}{\multirow{-20}{*}{\textbf{1}}}    & \multirow{-10}{*}{\textbf{MS}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{0.617}}       & \multicolumn{1}{c|}{\multirow{-10}{*}{0.038}}          & \multicolumn{1}{c|}{SA20*SA30}                             & -0.154                              & \multicolumn{1}{c|}{\multirow{-5}{*}{0.534}}       & \multicolumn{1}{c|}{\multirow{-10}{*}{0.136}}          & \multicolumn{1}{c|}{SA20*SA30}                             & 0.987                               \\ \hline
% \end{tabular}
% \label{tab:regression_model2a}
% \end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[h!]
\caption{A multiple regression model to predict RC and MS in normal and remote driving. The light gray coloured cells are the ones have not been included in the developed models. Significance is presented by  $^{***}P\le0.001$,$^{**}P\le0.01$, and $^{*}P\le0.05$.}
\begin{tabular}{|c|ccccc|ccccc|}
\hline
                               & \multicolumn{5}{c|}{}                                                                                                                                                                                                                                         & \multicolumn{5}{c|}{}                                                                                                                                                                                                                                         \\
                               & \multicolumn{5}{c|}{\multirow{-2}{*}{\textbf{Normal driving}}}                                                                                                                                                                                                & \multicolumn{5}{c|}{\multirow{-2}{*}{\textbf{Remote driving}}}                                                                                                                                                                                                \\ \cline{2-11} 
                               & \multicolumn{2}{c|}{}                                                                                & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{}                                      &                                  & \multicolumn{2}{c|}{}                                                                                & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{}                                      &                                  \\
\multirow{-4}{*}{}             & \multicolumn{2}{c|}{\multirow{-2}{*}{\textbf{R$^2$}}}                                                & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{pValue}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Predictors}}} & \multirow{-2}{*}{\textbf{Terms}} & \multicolumn{2}{c|}{\multirow{-2}{*}{\textbf{R$^2$}}}                                                & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{pValue}}} & \multicolumn{1}{c|}{\multirow{-2}{*}{\textbf{Predictors}}} & \multirow{-2}{*}{\textbf{Terms}} \\ \hline
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Intercept}                             & 1.857                            & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Intercept}                             & 1.510                            \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA11}                                  & 0.148                            & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA11}          & \cellcolor[HTML]{D0CECE}-        \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA12}                                  & -0.099                           & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA12}                                  & 0.341                            \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA21}                                  & 0.266                            & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA21}                                  & 0.068                            \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\multirow{-5}{*}{}}                & \multicolumn{1}{c|}{SA22}                                  & -1.150                           & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\multirow{-5}{*}{}}                & \multicolumn{1}{c|}{SA22}                                  & -0.167                           \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{\multirow{-6}{*}{\textbf{Calc.}}} & \multicolumn{1}{c|}{\multirow{-6}{*}{0.991}} & \multicolumn{1}{c|}{***}                               & \multicolumn{1}{c|}{SA31}                                  & -0.038                           & \multicolumn{1}{c|}{\multirow{-6}{*}{\textbf{Calc.}}} & \multicolumn{1}{c|}{\multirow{-6}{*}{0.901}} & \multicolumn{1}{c|}{***}                               & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA31}          & \cellcolor[HTML]{D0CECE}-        \\ \cline{2-3} \cline{5-8} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.000}                             & \multicolumn{1}{c|}{SA32}                                  & -0.044                           & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.001}                             & \multicolumn{1}{c|}{SA32}                                  & 0.306                            \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA12*SA32}                             & -0.197                           & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA12*SA32}                             & -0.212                           \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA22*SA31}                             & 0.199                            & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA22*SA31}     & \cellcolor[HTML]{D0CECE}-        \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA22*SA32}     & \cellcolor[HTML]{D0CECE}-        & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA22*SA32}                             & 0.088                            \\ \cline{5-6} \cline{10-11} 
\multirow{-11}{*}{\textbf{RC}} & \multicolumn{1}{c|}{\multirow{-5}{*}{\textbf{Adj.}}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{0.974}} & \multicolumn{1}{c|}{\multirow{-4}{*}{}}                & \multicolumn{1}{c|}{SA31*SA32}                             & 0.144                            & \multicolumn{1}{c|}{\multirow{-5}{*}{\textbf{Adj.}}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{0.828}} & \multicolumn{1}{c|}{\multirow{-4}{*}{}}                & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA31*SA32}     & \cellcolor[HTML]{D0CECE}-        \\ \hline
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{}                                  & \multicolumn{1}{c|}{Intercept}                             & -0.330                           & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{Intercept}                             & -2.873                           \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA11}          & \cellcolor[HTML]{D0CECE}-        & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA11}          & \cellcolor[HTML]{D0CECE}-        \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA12}          & \cellcolor[HTML]{D0CECE}-        & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA12}          & \cellcolor[HTML]{D0CECE}-        \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{\multirow{-4}{*}{}}                & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA21}          & \cellcolor[HTML]{D0CECE}-        & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{\multirow{-4}{*}{}}                & \multicolumn{1}{c|}{SA21}                                  & 1.030                            \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{\multirow{-5}{*}{\textbf{Calc.}}} & \multicolumn{1}{c|}{\multirow{-5}{*}{0.833}} & \multicolumn{1}{c|}{**}                                & \multicolumn{1}{c|}{SA22}                                  & -0.044                           & \multicolumn{1}{c|}{\multirow{-5}{*}{\textbf{Calc.}}} & \multicolumn{1}{c|}{\multirow{-5}{*}{0.966}} & \multicolumn{1}{c|}{**}                                & \multicolumn{1}{c|}{SA22}                                  & -0.084                           \\ \cline{2-3} \cline{5-8} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{l|}{0.010}                             & \multicolumn{1}{c|}{SA31}                                  & 0.304                            & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{0.016}                             & \multicolumn{1}{c|}{SA31}                                  & 0.848                            \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA32}                                  & 0.190                            & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA32}                                  & 0.709                            \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA21*SA31}     & \cellcolor[HTML]{D0CECE}-        & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}SA21*SA31}     & \cellcolor[HTML]{FFFFFF}-0.209   \\ \cline{5-6} \cline{10-11} 
                               & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}SA22*SA32}     & -0.089                           & \multicolumn{1}{c|}{}                                 & \multicolumn{1}{c|}{}                        & \multicolumn{1}{c|}{}                                  & \multicolumn{1}{c|}{SA22*SA32}                             & -0.126                           \\ \cline{5-6} \cline{10-11} 
\multirow{-10}{*}{\textbf{MS}} & \multicolumn{1}{c|}{\multirow{-5}{*}{\textbf{Adj.}}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{0.534}} & \multicolumn{1}{c|}{\multirow{-4}{*}{}}                & \multicolumn{1}{c|}{\cellcolor[HTML]{D0CECE}SA31*SA32}     & \cellcolor[HTML]{D0CECE}-        & \multicolumn{1}{c|}{\multirow{-5}{*}{\textbf{Adj.}}}  & \multicolumn{1}{c|}{\multirow{-5}{*}{0.881}} & \multicolumn{1}{c|}{\multirow{-4}{*}{}}                & \multicolumn{1}{c|}{SA31*SA32}                             & -0.111                           \\ \hline
\end{tabular}
\label{tab:regression_model2b}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
